Joint Near Field Uplink Communication and Localization Using Message Passing-Based Sparse Bayesian Learning

This work deals with the problem of uplink communication and localization in an integrated sensing and communication system, where users are in the near field (NF) of antenna aperture due to the use of high carrier frequency and large antenna arrays at base stations. We formulate joint NF signal detection and localization as a problem of recovering signals with a sparse pattern. To solve the problem, we develop a message passing based sparse Bayesian learning (SBL) algorithm, where multiple unitary approximate message passing (UAMP)-based sparse signal estimators work jointly to recover the sparse signals with low complexity. Simulation results demonstrate the effectiveness of the proposed method.

==> factorgraph.tex <==
%\draw[black, rounded corners] (-1.2,1.4) rectangle (4.4,-4.6);

%\draw[black, thick, dashed, rounded corners] (-1.2,1.8) rectangle (3.7,-3.8);
%
%\filldraw[white, dashed, rounded corners] (-0.9,1.4) rectangle (4,-4.2);
%\draw[black, thick, dashed, rounded corners] (-0.9,1.4) rectangle (4,-4.2);
%
\filldraw[gray!10, rounded corners] (0,1.9) rectangle (6.6,-2.5);
\draw[black!30, thick, rounded corners] (0, 1.9) rectangle (6.6,-2.5);

\filldraw[gray!10, rounded corners] (-0.6,1.2) rectangle (6,-3.2);
\draw[black!30, thick, rounded corners] (-0.6, 1.2) rectangle (6,-3.2);

\filldraw[gray!10, xslant=0.3] (-4.6,-0.4) rectangle (-1.6,-2.0);
\draw[black!30, thick, xslant=0.3, rounded corners] (-4.6,-0.4) rectangle (-1.6,-2.0);

\filldraw[gray!10, rounded corners] (7.9, 2) rectangle (10.5,-3.4);
\draw[black!30, thick, rounded corners] (7.9, 2) rectangle (10.5,-3.4);

\node[font=\normalsize] at (0.1,1) {$n=1$};
\node[font=\normalsize] at (0.4,1.7) {$N$};
\node[rotate=-45, font=\large] at (3,1.6) {$\boldsymbol{\vdots}$};

\node (fy1)[funnode, ] at (0,0) {};		
\node [above= -1mm of fy1] {$f_{\overline{\boldsymbol{y}}_1^n}$};	

%\node (vdot1)[below = 0mm of fy1]  {$\boldsymbol{\vdots}$};

\node (fyr)[funnode, below = 6mm of fy1] {};			
\node [above= -1mm of fyr] {$f_{\overline{\boldsymbol{y}}_l^n}$};	

%\node (vdot2)[below = 0mm of fyr]  {$\boldsymbol{\vdots}$};

\node (fyR)[funnode, below = 6mm of fyr] {};			
\node [above= -1.5mm of fyR] {$f_{\overline{\boldsymbol{y}}_L^n}$};	

\node (gamma) [factornode, left = 2.2cm of fyr] {$\gamma$};
\node (fgamma)[funnode, left = 6mm of gamma ] {};		
\node [above= -1mm of fgamma] {$f_{\gamma}$};	

\node (h1) [factornode, right = 6mm of fy1] {$\boldsymbol{h}_1^n$};
\node (hr) [factornode, right = 6mm of fyr] {$\boldsymbol{h}_l^n$};
\node (hR) [factornode, right = 6mm of fyR] {$\boldsymbol{h}_L^n$};


\node (fh1)[funnode, right = 6mm of h1 ] {};	
\node [above= -1mm of fh1] {$f_{\boldsymbol{h}_1^n}$};
\node (fhr)[funnode, right = 6mm of hr ] {};	
\node [above= -1mm of fhr] {$f_{\boldsymbol{h}_l^n}$};
\node (fhR)[funnode, right = 6mm of hR ] {};	
\node [above= -1mm of fhR] {$f_{\boldsymbol{h}_L^n}$};

\node (zn1) [factornode, right = 6mm of fh1] {$\boldsymbol{z}_1^n$};
\node (znl) [factornode, right = 6mm of fhr] {$\boldsymbol{z}_l^n$};
\node (znL) [factornode, right = 6mm of fhR] {$\boldsymbol{z}_L^n$};

\node (fz1)[funnode, right = 6mm of zn1 ] {};	
\node [above= -1mm of fz1] {$f_{\boldsymbol{z}_1^n}$};
\node (fzl)[funnode, right = 6mm of znl ] {};	
\node [above= -1mm of fzl] {$f_{\boldsymbol{z}_l^n}$};
\node (fzL)[funnode, right = 6mm of znL ] {};	
\node [above= -1mm of fzL] {$f_{\boldsymbol{z}_L^n}$};

\node (lambda1) [factornode, right = 2.6cm of fz1, yshift=6mm] {$\lambda_1$};
%\node (vdot3)[below = 6mm of lambda1]  {$\boldsymbol{\vdots}$};
\node (lambdam) [factornode, right = 2.6cm of fzl] {$\lambda_m$};
%\node (vdot4)[below = 6mm of lambdam]  {$\boldsymbol{\vdots}$};
\node (lambdaM) [factornode, right =2.6cm of fzL, yshift=-4mm] {$\lambda_M$};

\node (flambda1)[funnode, right = 6mm of lambda1 ] {};	
\node [above= -1mm of flambda1] {$f_{\lambda_1}$};
\node (flambdam)[funnode, right = 6mm of lambdam ] {};	
\node [above= -1mm of flambdam] {$f_{\lambda_m}$};
\node (flambdaM)[funnode, right = 6mm of lambdaM ] {};	
\node [above= -1mm of flambdaM] {$f_{\lambda_M}$};


\draw[thick] (fgamma) -- (gamma); 
\draw[thick] (gamma.east) -- (fy1.west);
\draw[thick] (gamma.east) -- (fyr.west);
\draw[thick] (gamma.east) -- (fyR.west);
\draw[thick] (fy1) -- (h1) -- (fh1);
\draw[thick] (fyr) -- (hr) -- (fhr);
\draw[thick] (fyR) -- (hR) -- (fhR);

\draw[dashed, thick] (gamma.east) -- ($(fy1.west) + (-0.3,0.6)$);
\draw[dashed, thick] (gamma.east) -- ($(fyr.west) + (-0.3,0.6)$);
\draw[dashed, thick] (gamma.east) -- ($(fyR.west) + (-0.3,0.6)$);

\draw[thick] (fh1) -- (zn1) -- (fz1); 
\draw[thick] (fhr) -- (znl) -- (fzl);
\draw[thick] (fhR) -- (znL) -- (fzL);

\draw[thick] (fz1.east) -- (lambda1.west); 
\draw[thick] (fz1.east) -- (lambdam.west); 
\draw[thick] (fz1.east) -- (lambdaM.west);
\draw[thick] (fzl.east) -- (lambda1.west); 
\draw[thick] (fzl.east) -- (lambdam.west); 
\draw[thick] (fzl.east) -- (lambdaM.west);
\draw[thick] (fzL.east) -- (lambda1.west); 
\draw[thick] (fzL.east) -- (lambdam.west); 
\draw[thick] (fzL.east) -- (lambdaM.west);

\draw[dashed] ($(fz1.east) + (0.45, 0.5)$) -- (lambda1.west);
\draw[dashed] ($(fzl.east) + (0.45, 0.5)$) -- (lambda1.west);
\draw[dashed] ($(fzL.east) + (0.45, 0.7)$) -- (lambda1.west);

\draw[dashed] ($(fz1.east) + (0.45, 0.5)$) -- (lambdam.west);
\draw[dashed] ($(fzl.east) + (0.45, 0.5)$) -- (lambdam.west);
\draw[dashed] ($(fzL.east) + (0.45, 0.7)$) -- (lambdam.west);

\draw[dashed] ($(fz1.east) + (0.45, 0.5)$) -- (lambdaM.west);
\draw[dashed] ($(fzl.east) + (0.45, 0.5)$) -- (lambdaM.west);
\draw[dashed] ($(fzL.east) + (0.45, 0.7)$) -- (lambdaM.west);

\draw[thick] (lambda1.east) -- (flambda1);
\draw[thick] (lambdam.east) -- (flambdam);
\draw[thick] (lambdaM.east) -- (flambdaM);

